PDPU: An Open-Source Posit Dot-Product Unit for Deep Learning Applications

Posit has been a promising alternative to the IEEE-754 floating point format for deep learning applications due to its better trade-off between dynamic range and accuracy. However, hardware implementation of posit arithmetic requires further exploration, especially for the dot-product operations dominated in deep neural networks (DNNs). It has been implemented by either the combination of multipliers and an adder tree or cascaded fused multiply-add units, leading to poor computational efficiency and excessive hardware overhead. To address this issue, we propose an open-source posit dot-product unit, namely PDPU, that facilitates resource-efficient and high-throughput dot-product hardware implementation. PDPU not only features the fused and mixed-precision architecture that eliminates redundant latency and hardware resources, but also has a fine-grained 6-stage pipeline, improving computational efficiency. A configurable PDPU generator is further developed to meet the diverse needs of various DNNs for computational accuracy. Experimental results evaluated under the 28nm CMOS process show that PDPU reduces area, latency, and power by up to 43%, 64%, and 70%, respectively, compared to the existing implementations. Hence, PDPU has great potential as the computing core of posit-based accelerators for deep learning applications.

==> 0-abstr.tex <==
\begin{abstract}
Posit has been an emerging hot-spot in deep learning applications due to its unique advantages over conventional floating point formats.
However, the hardware design based on posit remains to be explored, especially for the dot-product operation in deep neural networks (DNNs), which is still performed based on separate arithmetic operation unit, leading to poor computational efficiency and excessive hardware overhead.
By contrast, we propose an open-source mixed-precision posit dot-product unit, namely PDPU, to achieve resource-efficient and high-throughput dot-product for hardware deployment of DNNs.
PDPU features not only for its fused arithmetic that eliminates redundant latency and hardware resources, but also a highly configurable generator with scalability for various DNNs, according to accuracy requirements and dot-product size.
A 28nm ASIC implementation results in 43\% less area, 64\% less delay and 2.34$\times$ less power consumption than traditional discrete architectures. 
Further experiments also reveal the excellent performance of the proposed 6-stage pipeline and the flexibility of PDPU under different parameters.
\end{abstract}

==> 1-intro.tex <==
\section{Introduction} \label{sec:intro}
% Posit \cite{gustafson2017beating} is regarded as a drop-in replacement for traditional floating-point numbers due to its better trade-off between dynamic range and accuracy. 
\Rone{Posit \cite{gustafson2017beating} is regarded as a drop-in replacement for conventional IEEE 754 floating-point format \cite{2008ieee754} due to its better trade-off between dynamic range and accuracy.}
It has \Rone{attracted} increasing attention in many fields of applications \cite{shah2021dpu, tiwari2021peri, mallasen2022percival, neves2021reconfigurable}, especially \Rone{for those} involved with DNNs \cite{langroudi2018deep, carmichael2019deep, lu2020evaluations, wang2022pl}.

To facilitate hardware deployment of DNNs, several posit arithmetic units have been proposed: adder \cite{chaurasiya2018parameterized} \cite{jaiswal2018architecture}, multiplier \cite{zhang2020design, jaiswal2019pacogen, murillo2020customized} and fused multiply-add (FMA) unit \cite{zhang2019efficient, murillo2021energy, crespo2022unified}. 
However, to the best of our knowledge, there are few works discussing posit-based dot-product operations, which generally occupy most of computational workload for both training and inference tasks in DNNs \cite{lee2021resource}, e.g., there exists up to 724M and 3.9G multiply-accumulate (MAC) operations in AlexNet and ResNet50 \cite{sze2017efficient}, respectively, which are the decomposition of long dot-product operation in convolution layers and fully connected layers. 
It would introduce plenty of drawbacks if these operations are performed using the discrete architecture illustrated in Fig. \ref{fig:discrete}.
First, extensive redundant logic including complicated encoding and decoding process are retained in separate arithmetic unit, leading to an excessive hardware overhead and high latency. 
Besides, frequent rounding in intermediate operations may also cause a loss in accuracy. 
Furthermore, despite the great benefits of mixed-precision proved in DNNs \cite{micikevicius2017mixed}, off-the-shell discrete architecture do not support this strategy, resulting in a memory waste of data width.
% TODO

However, all the above challenges can be tackled by a fused mixed-precision dot-product unit (DPU), which is able to share common components among parallel inputs while decreasing unnecessary operations, aiming for an enhanced hardware efficiency and reduced latency. 
Fewer rounding also ensures higher accuracy at the same posit formats.
Therefore, it would be a better choice as a computing core in modern posit-based AI accelerators in deep learning applications.
% Therefore, DPU, earning benefits from fused arithmetic and mixed-precision compared with traditional discrete implementations, would be a better choice as a computing core in modern posit-based ai accelerator in DNNs.

% Compared with discrete architecture composed of separate units (as illustrated in Fig. \ref{fig:discrete}), a fused dot-product unit (DPU) brings strengths in both hardware resources and precision. First, it is able to share common components among parallel inputs while decreasing redundant logic including complicated encoding and decoding process of intermediate values, and thus contributes to an enhanced hardware efficiency and reduced latency. Meanwhile, fewer rounding in fused arithmetic ensures higher accuracy at the same posit formats. 

% First, the rounding process is involved just once before output, and hence, the loss of intermediate operations is reduced. Second, fused arithmetic can share components in parallel inputs and decrease redundant logic, which contributes to a reduced area and delay. Furthermore, despite the great benefits of mixed-precision proved in DNNs\cite{micikevicius2017mixed}, off-the-shell posit-based arithmetic units\cite{jaiswal2019pacogen}\cite{zhang2019efficient} do not support this strategy, which may lead to a larger bit-width to achieve the same precision. 

\begin{figure}[t]
	\centering
	\subfigure[]{
    	\begin{minipage}{0.4\linewidth}
    		\centering
    		\includegraphics[width=\textwidth]{figs/discrete_1.pdf}
    	\end{minipage}
	}
	\subfigure[]{
    	\begin{minipage}{0.42\linewidth}
    		\centering
    		\includegraphics[width=\textwidth]{figs/discrete_2.pdf}
    	\end{minipage}
	}
	\caption{Discrete dot-product architecture implemented by (a) multipliers and adders or (b) FMA units}
	\label{fig:discrete}
\end{figure}

In this paper, we present PDPU, an open-source\footnote{The whole work will be available on GitHub upon the acceptance.} mixed-precision posit dot-product unit, to perform the universal dot-product operations in DNNs efficiently. 
It introduces the following contributions and features:

% In this paper, a fused posit DPU with mixed-precision support is proposed to tackle above challenges. It is highly parameterized with configurable posit format and dot-product size. Also, the unit avoids the huge cost of exact accumulation using quire by supporting custom alignment width. It introduces the following contributions and features:
\begin{enumerate}
    \item PDPU takes full advantage of fused dot-product arithmetic and mixed-precision based on posit, achieving significant reduction of up to 43\%, 64\% and 70\% in area, latency and power compared with conventional discrete architecture. Memory footprint is also decreased over 50\% than that based on traditional FP32 format. 
    \item PDPU is implemented as a configurable DPU generator, supporting arbitrary posit formats, dot-product size and alignment width. The excellent flexibility enable its adaptation to different DNNs. 
    \item PDPU has been optimized with a fine-grained 6-stage pipeline, to minimize the critical path for higher computational efficiency. Its performance has been demonstrated by breaking down the latancy and resources at each stage.
\end{enumerate}

% 篇幅紧张
% The rest of the paper is organized as follows: Section~\ref{sec:bkg} presents the posit format as well as its potential in DNNs. The proposed open-source posit DPU is presented in Section III. Section IV presents the synthesis results of our architecture and comparisons with traditional designs. Finally, the work is summarized in Section V.

==> 2-bkg.tex <==
\section{Background}\label{sec:bkg}
Posit is first introduced by Professor Gustafson in \cite{gustafson2017beating}, and then many works \cite{lindstrom2018universal, de2019posits, murillo2020deep} have proved its advantages over traditional floating-point formats in DNNs. 
% It is defined by word size $n$ and exponent size $es$, consisting of sign, regime, exponent and mantissa, as described in Fig. \ref{fig:2_posit_format}. 
As described in Fig. \ref{fig:2_posit_format}, a posit number is defined by the word size $n$ and exponent size $es$, which consists of 4 fields, namely sign, regime, exponent and mantissa.
Regime is composed of $m$ consecutive identical bits $r$ and an opposite bit $\overline{r}$, indicating a scale factor of $2^{k\cdot 2^{es}}$, where $k=-m$ if $r$ is 0 and $m-1$ if $r$ is 1, respectively. 
Exponent and mantissa fields are sequentially distributed after regime, occupying the remaining bit positions, since the bit-width of regime varies under different $k$. 
A posit number is decoded as follows:
\begin{equation}
    \label{eq:2_posit}
    p = \left\{
    \begin{array}{lc}
         \pm 0,& 000...000, \\
         \pm \infty,& 100...000, \\
         (-1)^s\times 2^{k\cdot 2^{es}}\times 2^{e_p}\times 1.m_p,& otherwise,
    \end{array}
    \right.
\end{equation}
where $s$, $e_p$, $m_p$ represents sign, exponent and mantissa value respectively. 
And if negative, the data need to be complemented first before decoding.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.85\linewidth]{figs/Posit数值格式结构.pdf}
    \caption{Format of posit number}
    \label{fig:2_posit_format}
\end{figure}

As there are no posit subnormal or NaN representations, the handling of exceptional cases is simplified greatly than in IEEE 754 format.
Furthermore, its non-uniform encoding manner contributes to a symmetrical tapered accuracy distribution, which is almost consistent with the network parameters distribution of deep learning. 
The feature is illustrated in Fig. \ref{fig:2_decimal_accuracy}, where decimal accuracy of posit fits the activations of the first convolution layer of ResNet18 well, implying the potential of substituting low-width posit for high-width FP formats.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/precision_distribution_v2.pdf}
    \caption{Tapered accuracy of posit fits the DNN data distribution}
    \label{fig:2_decimal_accuracy}
\end{figure}

Despite the immense advantages, the research of posit-based hardware design for deep learning applications is far from sufficient. 
For example, several existing posit-based arithmetic units \cite{jaiswal2019pacogen} \cite{zhang2019efficient} do not support mixed-precision computation, and fused dot-product operation is less discussed. 
Fortunately, PDPU proposed in this work is capable to deal with the above challenges, promising for real-life DNN applications.

% However, the research on posit DPU is far from sufficient compared with the FP fused dot product unit, which has been well discussed in the literature\cite{saleh2008floating}\cite{tao2013correctly}\cite{sohn2016fused}\cite{kaul2019optimized}. Motivated by the above fact, this work presents PDPU, a highly configurable open-source fused posit DPU, capable of supporting any custom posit format and dot-product size.

==> 5-concls.tex <==
\section{Conclusion}\label{sec:concls}
In this work, we have presented PDPU, a configurable open-source posit dot-product unit to perform efficient dot-product operations in deep learning applications.
It provides higher computational performance and hardware efficiency, benefiting from fused and mixed-precision arithmetic.
The capability of supporting arbitrary posit formats, dot-product size and alignment width allows PDPU to be embedded as computing unit for various DNNs.
A fine-grained 6-stage pipelined is also proposed to further improve the thoughput of PDPU.
Compared with corresponding discrete implementation at the same model accuracy, our design achieves a reduction of 43\%, 60\%, and 70\% in terms of area, latency, and power, respectively.
